Development of an early warning method incorporating pre-supernova neutrino light curves

Massive stars ($M>8\mathrm{M_\odot}$) emit neutrinos known as pre-supernova (pre-SN) neutrinos through thermal and nuclear interactions for cooling the stellar core during the final stage of stellar evolution. Real-time monitoring of their pre-SN neutrino interaction rate offers a crucial opportunity to issue an early warning to a core-collapse supernova. Some neutrino detectors, including KamLAND and Super-Kamiokande already operate pre-SN alarm systems based on a statistically significant excess of the observed event rate over the expected background. To improve alarm sensitivity, an alarm method which incorporates the time evolution of the observed pre-SN neutrino event rate was proposed in A. Sheshukov et al. (2021). We evaluate the performance of the light-curve likelihood approach under realistic KamLAND and SK operating conditions, including realistic background rates, global false-alarm-rate calibration, and the combined alarm. The results demonstrate a significant improvement in the alarm time and distance compared to the conventional rate-only method, while maintaining the same false alarm rate.

==> AuthorList.tex <==
%AutherList (A-Z, fammily name)
\author{K.Saito}
\affiliation{Research Center for Neutrino Science, Tohoku University, Sendai 980-8578, Japan}
\email{saito@awa.tohoku.ac.jp}
\author{M.Eizuka}
\affiliation{Research Center for Neutrino Science, Tohoku University, Sendai 980-8578, Japan}
\email{}
\author{Z.Hu}
%previous affiliation
\affiliation{Department of Physics, Kyoto University, Kyoto, Kyoto 606-8502, Japan}
\affiliation{Ecole Polytechnique, IN2P3-CNRS, Laboratoire Leprince-Ringuet, F-91120 Palaiseau, France}
\email{}
\author{K.Ichimura}
\affiliation{Research Center for Neutrino Science, Tohoku University, Sendai 980-8578, Japan}
\email{}
\author{M.Ikeda}
\affiliation{Kamioka Observatory, Institute for Cosmic Ray Research, University of Tokyo, Kamioka, Gifu 506-1205, Japan}
\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study, University of Tokyo, Kashiwa, Chiba 277-8583, Japan}
\email{}
\author{K.Ishidoshiro}
\affiliation{Research Center for Neutrino Science, Tohoku University, Sendai 980-8578, Japan}
\email{}
\author{N.Kawada}
\affiliation{Research Center for Neutrino Science, Tohoku University, Sendai 980-8578, Japan}
\email{}
\author{L.N.Machado}
\affiliation{School of Physics and Astronomy, University of Glasgow, Glasgow, Scotland, G12 8QQ, United Kingdom}
\email{}
\author{Ll.Marti}
\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study, University of Tokyo, Kashiwa, Chiba 277-8583, Japan}
\email{}
\author{K.Mikami}
\affiliation{Research Center for Neutrino Science, Tohoku University, Sendai 980-8578, Japan}
\email{}
\author{K.Tachibana}
\affiliation{Research Center for Neutrino Science, Tohoku University, Sendai 980-8578, Japan}
\email{}
\author{R.A.Wendell}
\affiliation{Department of Physics, Kyoto University, Kyoto, Kyoto 606-8502, Japan}
\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study, University of Tokyo, Kashiwa, Chiba 277-8583, Japan}
\email{}
